Interpretable Clinical Classification with Kolmogorov-Arnold Networks

The increasing use of machine learning in clinical decision support has been limited by the lack of transparency of many high-performing models. In clinical settings, predictions must be interpretable, auditable, and actionable. This study investigates Kolmogorov-Arnold Networks (KANs) as intrinsically interpretable alternatives to conventional black-box models for clinical classification of tabular health data, aiming to balance predictive performance with clinically meaningful transparency. We introduce two KAN-based models: the Logistic KAN, a flexible generalization of logistic regression, and the Kolmogorov-Arnold Additive Model (KAAM), an additive variant that yields transparent symbolic representations through feature-wise decomposability. Both models are evaluated on multiple public clinical datasets and compared with standard linear, tree-based, and neural baselines. Across all datasets, the proposed models achieve predictive performance comparable to or exceeding that of commonly used baselines while remaining fully interpretable. Logistic-KAN obtains the highest overall ranking across evaluation metrics, with a mean reciprocal rank of 0.76, indicating consistently strong performance across tasks. KAAM provides competitive accuracy while offering enhanced transparency through feature-wise decomposability, patient-level visualizations, and nearest-patient retrieval, enabling direct inspection of individual predictions. KAN-based models provide a practical and trustworthy alternative to black-box models for clinical classification, offering a strong balance between predictive performance and interpretability for clinical decision support. By enabling transparent, patient-level reasoning and clinically actionable insights, the proposed models represent a promising step toward trustworthy AI in healthcare (code: https://github.com/Patricia-A-Apellaniz/classification_with_kans).

==> math_commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath,amsfonts,bm}
\RequirePackage{suffix}

% punctuation of equations, see for example the first answer in
% https://www.reddit.com/r/LaTeX/comments/5xnzg7/correct_grammar_for_putting_an_equation/
\newcommand{\equationPunctuation}[1]{\,{#1}}

%% Bold greek letters
\newcommand{\thetab}{{\boldsymbol{\theta}}}
\newcommand{\betab}{{\boldsymbol{\beta}}}
\newcommand{\pib}{{\boldsymbol{\pi}}}
\newcommand{\taub}{{\boldsymbol{\tau}}}
\newcommand{\psib}{{\boldsymbol{\psi}}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\omegab}{{\boldsymbol{\omega}}}
\newcommand{\etab}{{\boldsymbol{\eta}}}
\newcommand{\sigmab}{{\boldsymbol{\sigma}}}
\newcommand{\epsilonb}{{\boldsymbol{\epsilon}}}

\newcommand{\Thetab}{{\boldsymbol{\Theta}}}

\newcommand{\distribution}[1][]{\ensuremath{{P}_{#1}}\xspace}
\newcommand{\cumulative}[1][]{\ensuremath{F_{#1}}\xspace}
\newcommand{\empcumulative}[1][]{\ensuremath{\hat F_{#1}}\xspace}
\newcommand{\pushforward}[2]{{#1}_{\#} {#2}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclarePairedDelimiter{\Ebrackets}{[}{]}
\newcommand{\Expect}[2][]{\E_{#1}\Ebrackets{#2}}
\WithSuffix\newcommand\Expect*[2][]{\E_{#1}\Ebrackets*{#2}}

\DeclareMathOperator{\V}{\mathbb{V}}
\newcommand{\Var}[2][]{\V_{#1}\Ebrackets{#2}}

\newcommand{\normal}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\uniform}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\categorical}{\ensuremath{\operatorname{Cat}}\xspace}
\newcommand{\bernoulli}{\ensuremath{\operatorname{Bern}}\xspace}
\newcommand{\binomial}{\ensuremath{\operatorname{Bin}}\xspace}
\newcommand{\lognormal}{\ensuremath{\operatorname{Log-normal}}\xspace}
\newcommand{\poisson}{\ensuremath{\operatorname{Poiss}}\xspace}
\newcommand{\exponentialdistribution}{\ensuremath{\operatorname{Exp}}\xspace}
\newcommand{\betadistribution}{\ensuremath{\operatorname{Beta}}\xspace}
\newcommand{\weibulldistribution}{\ensuremath{\operatorname{Weibull}}\xspace}

\newcommand{\identity}{\ensuremath{\mI}}
\newcommand{\indicator}[1]{\ensuremath{\mathbf{1}_{\{#1\}}}}
\newcommand{\ones}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\zeroes}{\ensuremath{\mathbf{0}}\xspace}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\med}{med}
\DeclareMathOperator*{\std}{std}

\let\cossim\cos

%%%%%%

\usepackage{suffix}
\usepackage{xparse}
\usepackage{mathtools}

%%%%
\def\rL{{\textnormal{L}}}
\def\rvL{{\mathbf{L}}}
\def\ervL{{\textnormal{L}}}

\def\rM{{\textnormal{M}}}
\def\rvM{{\mathbf{M}}}
\def\ervM{{\textnormal{M}}}

\def\vT{\bm{T}}
\def\vF{\bm{F}}
\def\vR{\bm{R}}
\def\vU{\bm{U}}
\def\rU{{\textnormal{U}}}
\def\rvU{{\mathbf{U}}}
\def\ervU{{\textnormal{U}}}
%%%%

\newcommand{\tensor}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\vec}{\operatorname{vec}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\Gmat}{\mathrm{G}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\He}{\mathrm{H}}
\newcommand{\HeCal}{\mathcal{H}}
%\newcommand{\diff}{\mathrm{d}}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\average}[1]{\overline{ #1 }}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\jac}{\mathrm{J}}
\newcommand{\lin}[1]{\left\langle #1 \right\rangle}

\newcommand{\nablasquaredsub}[1]{
  \nabla^{\kern -.0em \raise.1em\hbox{\tiny$2$}} {\kern -.6em \raise-.1em\hbox{\tiny$#1$}}{}
}
\newcommand{\nablasub}[1]{
  \nabla {\kern -.2em \raise-.1em\hbox{\tiny$#1$}}{}
}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}\xspace}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}\xspace}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\bfseries \color{maincolor} (a)}\xspace}
\newcommand{\captionb}{{\bfseries \color{maincolor}  (b)}\xspace}
\newcommand{\captionc}{{\bfseries \color{maincolor}  (c)}\xspace}
\newcommand{\captiond}{{\bfseries \color{maincolor}  (d)}\xspace}


% Added by me (@Adrian) to be consinstent when I do listings
\newcommand{\itemi}{{\bfseries \color{maincolor} i)}\xspace}
\newcommand{\itemii}{{\bfseries \color{maincolor} ii)}\xspace}
\newcommand{\itemiii}{{\bfseries \color{maincolor} iii)}\xspace}
\newcommand{\itemiv}{{\bfseries \color{maincolor} iv)}\xspace}
\newcommand{\itemv}{{\bfseries \color{maincolor} v)}\xspace}
\newcommand{\itemvi}{{\bfseries \color{maincolor} vi)}\xspace}
\newcommand{\itemvii}{{\bfseries \color{maincolor} vii)}\xspace}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vnu{{\bm{\nu}}}
\def\vtheta{{\bm{\theta}}}
\def\vgamma{{\bm{\gamma}}}
\def\vdelta{{\bm{\delta}}}
\def\vDelta{{\bm{\Delta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vehat{\bm{\hat{e}}}
\def\vetilde{\bm{\tilde{e}}}
\def\vell{{\bm{\ell}}}
\def\vf{{\bm{f}}}
\def\vfhat{{\bm{\hat{f}}}}
\def\vg{{\bm{g}}}
\def\vgtilde{\bm{\tilde{g}}}
\def\vghat{\bm{\hat{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vmhat{{\bm{\hat{m}}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vphi{{\bm{\phi}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vstilde{\bm{\tilde{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vvhat{{\bm{\hat{v}}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vytilde{{\bm{\tilde{y}}}}
\def\vyhat{{\bm{\hat{y}}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evyhat{{\hat{y}}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mGtilde{\bm{\tilde{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mWhat{{\bm{\hat{W}}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mPi{{\bm{\Pi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\mStilde{\bm{\tilde{\mS}}}
\def\mGtilde{\bm{\tilde{\mG}}}
\def\mGoverline{{\bm{\overline{G}}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sYhat{{\hat{\mathbb{Y}}}}
\def\sZ{{\mathbb{Z}}}
% Blackboard Greek characters: https://tex.stackexchange.com/a/3260
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\def\sOmega{{\mathbbold{\Omega}}}
\def\sPhi{{\mathbbold{\Phi}}}
\def\sTheta{{\mathbbold{\Theta}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}
\def\emPi{{\Pi}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdf}{p}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\mathrm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\mathrm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\mathrm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\ifcsname laplace\endcsname%
    \renewcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\else%
    \newcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\fi

%\newcommand{\E}{\mathbb{E}}
%\DeclareMathOperator{\E}{\mathbb{E}}

\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\onehot}{\mathrm{onehot}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\DeclareMathOperator{\KL}{KL}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}_{#1}}\xspace}}
% \newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}_{#1}}\xspace}}
% \newcommand{\children}[1]{{\ensuremath{\mathrm{ch}_{#1}}\xspace}}

\newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}(#1)}\xspace}}
\newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}(#1)}\xspace}}
\newcommand{\children}[1]{{\ensuremath{\mathrm{ch}(#1)}\xspace}}

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator*{\maximize}{maximize}

\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator{\vmap}{vmap}
\DeclareMathOperator{\reshape}{reshape}
%\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecspan}{span}
\DeclareMathOperator{\overlap}{overlap}
\DeclareMathOperator{\Cat}{Cat}

%%%%% NEW MATH DEFINITIONS %%%%%
\newcommand{\grad}[1]{\ensuremath{\nabla_{\!{#1}}}}
\newcommand{\naturalgrad}[1]{\ensuremath{\tilde{\nabla}_{\!{#1}}}}
\newcommand{\gradsquared}[1]{\ensuremath{\nabla_{\!{#1}}^{2}}}
\newcommand{\hess}[1]{\ensuremath{\mathrm{H}_{#1}}}

\newcommand{\Dtrain}{\ensuremath{\sD_{\mathrm{train}}}}
\newcommand{\Dtest}{\ensuremath{\sD_{\mathrm{test}}}}
\newcommand{\Dvalid}{\ensuremath{\sD_{\mathrm{valid}}}}


% || for KLDivergence
\DeclarePairedDelimiterX{\KLdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\KLdiv}{\KL\KLdivx}

\NewDocumentCommand{\giventhat}{O{\;|} m m}{#2#1\;#3}

\let\ab\allowbreak


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> my_commands.tex <==

%%% Colors
\colorlet{idcolor}{greendark}
\colorlet{unidcolor}{SBred}
\colorlet{hiddencolor}{gray}

\newcommand{\maincolor}{\textcolor{maincolor}{blue}\xspace}
\newcommand{\Maincolor}{\textcolor{maincolor}{Blue}\xspace}
\let\firstcolor\maincolor
\let\Firstcolor\Maincolor
\newcommand{\secondcolor}{\textcolor{secondcolor}{red}\xspace}
\newcommand{\Secondcolor}{\textcolor{secondcolor}{Red}\xspace}

%%% Boxes

\newtcolorbox{takeaway}{
    colback=maincolor!5!white, colframe=maincolor!75!black
}

%%% Text

\newcommand{\methodname}[1]{\texttt{\small #1}}


%%%

\newcommand{\oursIcon}{\faMicrochip\xspace}
% \newcommand{\ours}{TORO\xspace} % TODO change
% \newcommand{\Ours}{TORO\xspace}
\newcommand{\ours}{{xx}\xspace} % TODO change
\newcommand{\Ours}{{xx}\xspace}



\newcommand{\eqcomment}[1]{\text{[\textit{#1}]}}

%\renewcommand{\itemi}{\textit{i)}\xspace}
%\renewcommand{\itemii}{\textit{ii)}\xspace}
%\renewcommand{\itemiii}{\textit{iii)}\xspace}
%\renewcommand{\itemiv}{\textit{iv)}\xspace}
%\renewcommand{\itemv}{\textit{v)}\xspace}
%\newcommand{\itemvi}{\textit{vi)}\xspace}
%\newcommand{\itemvii}{\textit{vii)}\xspace}

%%% SYMBOLS

\newcommand{\kanlayer}{\ensuremath{\phi}\xspace}
\newcommand{\kanoutlayer}{\ensuremath{\Phi}\xspace}
\newcommand{\kan}{\ensuremath{\boldsymbol\Phi}\xspace}
\newcommand{\ELBO}{\ensuremath{\mathcal{L}}\xspace}

\newcommand{\splinecoef}{\ensuremath{w_s}\xspace}
\newcommand{\splinebiascoef}{\ensuremath{w_b}\xspace}
\newcommand{\weight}{\ensuremath{\lambda}\xspace}

%\let\pred\tilde
\renewcommand{\cond}[1]{{|{#1}}}
\newcommand{\pred}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\factual}[1]{\ensuremath{{#1}^\text{\normalfont{f}}}}
\newcommand{\cfactual}[1]{\ensuremath{{#1}^\text{\normalfont{cf}}}}

\newcommand{\indexone}{\ensuremath{i}\xspace}
\newcommand{\indextwo}{\ensuremath{j}\xspace}
\newcommand{\indexthree}{\ensuremath{q}\xspace}
\newcommand{\indexfour}{\ensuremath{k}\xspace}
\newcommand{\indexlayer}{\ensuremath{l}\xspace}
\newcommand{\indexfive}{\ensuremath{r}\xspace}
\newcommand{\indexsix}{\ensuremath{s}\xspace}

\newcommand{\nLayers}{\ensuremath{L}\xspace}

\newcommand{\query}{\ensuremath{Q}\xspace}

\newcommand{\doop}{\text{do}}


\newcommand{\scmfamily}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\scm}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\graph}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\func}[1][]{\ensuremath{f_{#1}}\xspace}
\newcommand{\funcb}[1][]{\ensuremath{\mathbf{g}_{#1}}\xspace}
\newcommand{\predfuncb}[1][]{\ensuremath{{\pred{\mathbf{f}}}_{#1}}\xspace}


% \newcommand{\varparents}[2][\varobs]{\ensuremath{{#1}_\parents{#2}}\xspace}
\newcommand{\varparents}[2][\varobs]{\ensuremath{\parents{#2}}\xspace}
% \newcommand{\varchildren}[2][\varobs]{\ensuremath{{#1}_\children{#2}}\xspace}
\newcommand{\varchildren}[2][\varobs]{\ensuremath{\children{#2}}\xspace}

\newcommand{\edist}{\ensuremath{\tilde{p}}\xspace}

\newcommand{\outcome}{\ensuremath{\rvy}\xspace}
\newcommand{\treatment}{\ensuremath{\rvt}\xspace}
\newcommand{\covariates}
{\ensuremath{\rvx}\xspace}
\newcommand{\covariate}
{\ensuremath{\text{x}}\xspace}
\newcommand{\latent}{\ensuremath{\rvz}\xspace}
\newcommand{\exogenous}{\ensuremath{\rvu}\xspace}

% \newcommand{\timepoint}{\ensuremath{\tau}\xspace}
% \newcommand{\timevar}{\ensuremath{\taub}\xspace}

\newcommand{\ite}{\ensuremath{\tau_\indexone}\xspace}
\newcommand{\cate}[1]{\ensuremath{\tau}(#1)\xspace}
\newcommand{\ate}{\ensuremath{\tau}\xspace}
\newcommand{\hcate}[1]{\ensuremath{\hat{\tau}}(#1)\xspace}


\newcommand{\hazard}{\ensuremath{h}\xspace}
\newcommand{\survival}{\ensuremath{S}\xspace}

\newcommand{\dataset}{\ensuremath{\mathcal{D}}\xspace}

\newcommand{\samplecov}{\ensuremath{\vx}\xspace}
\newcommand{\samplecovi}{\ensuremath{x}\xspace}
\newcommand{\samplelatent}{\ensuremath{\vz}\xspace}
\newcommand{\samplelatenti}{\ensuremath{z}\xspace}
\newcommand{\sampletreat}{\ensuremath{t}\xspace}
\newcommand{\sampletreati}{\ensuremath{t}\xspace}
\newcommand{\sampleoutcome}{\ensuremath{y}\xspace}
\newcommand{\sampleoutcomei}{\ensuremath{y}\xspace}

\newcommand{\samplekan}{\samplelatenti}

\newcommand{\covspace}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\treatmentspace}{\ensuremath{\mathcal{T}}\xspace}

\newcommand{\numtreatments}{\ensuremath{K}\xspace}

% \newcommand{\obssize}{\ensuremath{{D_\rvx}}\xspace}
\newcommand{\covsize}{\ensuremath{{D}}\xspace}
\newcommand{\latentsize}{{\ensuremath{\covsize_\latent}}\xspace}
\newcommand{\samplesize}{\ensuremath{N}\xspace}
\newcommand{\allsize}{\ensuremath{{D_\rvv}}\xspace}
\newcommand{\proxysize}{\ensuremath{{S}}\xspace}

\newcommand{\leftedge}{L\xspace}
\newcommand{\rightedge}{R\xspace}
\newcommand{\presence}[1]{\textcolor{firstcolor}{#1}}
\newcommand{\absence}[1]{\textcolor{secondcolor}{#1}}

\newcommand{\pozero}{\ensuremath{\mu_0}\xspace}
\newcommand{\hpozero}{\ensuremath{\hat{\mu}_0}\xspace}
\newcommand{\poone}{\ensuremath{\mu_1}\xspace}
\newcommand{\hpoone}{\ensuremath{\hat{\mu}_1}\xspace}
\newcommand{\pot}{\ensuremath{\mu_\sampletreati}\xspace}
\newcommand{\hpot}{\ensuremath{\hat{\mu}_\sampletreati}\xspace}
\newcommand{\propensity}{\ensuremath{e}\xspace}
\newcommand{\hpropensity}{\ensuremath{\hat{\propensity}}\xspace}
\newcommand{\hpo}{\ensuremath{\hat{\mu}}\xspace}

\newcommand{\score}{\ensuremath{s}\xspace}
\newcommand{\threshold}{\ensuremath{\Gamma}\xspace}
\newcommand{\budget}{\ensuremath{\Lambda}\xspace}

\newcommand{\significancelevel}{\ensuremath{\alpha}\xspace}
\newcommand{\regularization}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\representationspace}{\ensuremath{\boldsymbol\Delta}\xspace}


==> tikz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIBRARIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
    shapes,
    pgfplots.groupplots,
    shadings,
    calc,
    arrows,
    backgrounds,
    colorbrewer,
    shadows.blur,
    external,
    shapes,
    shapes.arrows,
    shapes.symbols,
    arrows.meta,
    positioning, 
    decorations.pathreplacing,
    intersections,
    cd,
    scopes,
    babel, % otherwise there is an error when importing spanish in babel
    fit % For extending the bounding box
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STYLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\tikzset{every picture/.style={->, shorten >=1pt, thick}}

% in preamble
\tikzcdset{
    nodes={anchor=center},
    arrow style=tikz,
    diagrams={>={Stealth[scale=0.8]}},
%    diagrams={>={Straight Barb[scale=0.8]}},
}

% \tikzstyle{main node}=[circle,draw,font=\sffamily\Large\bfseries]
\tikzstyle{main node}=[circle,draw,font=\sffamily\small,inner sep=0pt, outer sep=0pt, minimum size=5mm]
\tikzstyle{observed}=[style=main node, fill=gray!25]
\tikzstyle{hidden}=[style=main node, fill=white, dashed, draw=black!40, text=black!60]
\tikzstyle{hiddenarrow}=[dashed, draw=black!40]
\tikzstyle{realobs}=[style=main node,  ellipse]
\tikzstyle{realhidden}=[style=hidden, ellipse]
\tikzstyle{fairnessobs} = [style=main node, ellipse, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzstyle{fairnesshidden} = [style=main node, ellipse, fill=white, dashed, draw=black!60, text=black!60, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzset{
    given variable/.style = {
        draw=none, outer sep=0pt, inner sep=0pt, "#1"{yshift=-5pt}
    }
}

\tikzstyle{identifiable}=[draw=idcolor, very thick]
\tikzstyle{nonidentifiable}=[draw=unidcolor, very thick]


\tikzstyle{block} = [rectangle, draw, minimum width=0.5 cm, minimum height=1.5cm]
\tikzstyle{cir} = [circle, draw, minimum size=0.3cm]
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, aspect=2.5, minimum width=3cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{hexa} = [trapezium, trapezium left angle=60, trapezium right angle=120, draw,  
      minimum width=2cm, minimum height=0.5cm]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\irregularcircle[2]{% radius, irregularity
    \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
    +(0:\len pt)
    \foreach \a in {10,20,...,350}{
        \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
        -- +(\a:\len pt)
    } -- cycle
}


\pgfdeclareplotmark{mystar}{
    \node[star,star point ratio=2.25,minimum size=6pt,
    inner sep=0pt,draw=black,solid,fill=red] {};
}

% Optional: tighter spacing inside nodes
\newcommand{\nodew}{50mm}  % tweak node width
